To Fold or Not to Fold: a Necessary and Sufficient Condition on Batch-Normalization Layers Folding

Batch-Normalization (BN) layers have become fundamental components in the evermore complex deep neural network architectures. Such models require acceleration processes for deployment on edge devices. However, BN layers add computation bottlenecks due to the sequential operation processing: thus, a key, yet often overlooked component of the acceleration process is BN layers folding. In this paper, we demonstrate that the current BN folding approaches are suboptimal in terms of how many layers can be removed. We therefore provide a necessary and sufficient condition for BN folding and a corresponding optimal algorithm. The proposed approach systematically outperforms existing baselines and allows to dramatically reduce the inference time of deep neural networks.

==> tables/processing_time.tex <==
\begin{table}[!t]
\caption{Comparison of runtime reduction (run-T) and processing time (proc-T) in seconds, on different hardware and different architectures trained on Cifar10 and ImageNet.}
\label{tab:processing_time}
\centering
\setlength\tabcolsep{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{c|c|c|c|c}
\hline
& \multicolumn{2}{c|}{Intel m3} & \multicolumn{2}{c}{Intel i9-9900K}\\
\cline{2-5}
Model & run-T & proc-T & run-T & proc-T \\
\hline
\hline
ResNet 20 & 35.04 & 1.94 & 38.85 & 0.45 \\
ResNet 56 & 50.97 & 3.88 & 49.37 & 1.14\\
ResNet 110 & 54.36 & 11.98 & 51.20 & 2.15\\
ResNet 164 & 39.20 & 16.28 & 48.16 & 3.05\\
\hline
MobileNet & 29.01 & 12.48 & 27.76 & 1.84\\
\hline
ResNet 50 & 6.48 & 22.80 & 18.54 & 3.83\\
ResNet 101 & 10.34 & 43.90 & 16.77 & 6.59\\
ResNet 152 & 21.31 & 97.46 & 17.82 & 10.04\\
\hline
EfficientNet B0 & 18.27 & 11.53 & 20.74 & 3.60\\
EfficientNet B1 & 35.95 & 23.50 & 20.51 & 5.35\\
EfficientNet B5 & 21.38 & 251.34 & 11.80 & 37.87\\
\hline
\end{tabular}
\end{table}
